BEV-Seg: Bird's Eye View Semantic Segmentation Using Geometry and Semantic Point Cloud

Bird's-eye-view (BEV) is a powerful and widely adopted representation for road scenes that captures surrounding objects and their spatial locations, along with overall context in the scene. In this work, we focus on bird's eye semantic segmentation, a task that predicts pixel-wise semantic segmentation in BEV from side RGB images. This task is made possible by simulators such as Carla, which allow for cheap data collection, arbitrary camera placements, and supervision in ways otherwise not possible in the real world. There are two main challenges to this task: the view transformation from side view to bird's eye view, as well as transfer learning to unseen domains. Existing work transforms between views through fully connected layers and transfer learns via GANs. This suffers from a lack of depth reasoning and performance degradation across domains. Our novel 2-staged perception pipeline explicitly predicts pixel depths and combines them with pixel semantics in an efficient manner, allowing the model to leverage depth information to infer objects' spatial locations in the BEV. In addition, we transfer learning by abstracting high-level geometric features and predicting an intermediate representation that is common across different domains. We publish a new dataset called BEVSEG-Carla and show that our approach improves state-of-the-art by 24% mIoU and performs well when transferred to a new domain.

==> content/notes.tex <==
\section{introduction notes}



autonomous vehicle
av sensors
discuss about lidar, while provide valuable and accurate 3d information, expensive, sparse
av pipelines: perception, planning, prediction, control
discuss about planning representation
the use of simulatror provide cheap lots of data
to transfer learning from simulator, the use of domain adaptation



contributions:
-put together a perception pipeline that better incorporate depth information, utilize geometry, and various other tasks such as semantic segmentation, depth estimation to predict bird eyes' segmentation
-beat state of the art by 20 to 30 pct miou
-provide an alternate intermediate representation that is more robust and agnostic to sensor type and environment, experimentally show that this allows for better transfer learning
-release a new Carla dataset with rich variation in weather, town, and traffic congestion

----
\paragraph{Bird's Eye View}  In the cases of many 3D object detection models, LIDAR point clouds are first projected onto a 2D BEV with channels encoding intensities, densities, or levels of height \cite{beltran2018birdnet}. BEV is also often served as the representation at which features derived from different mode of input data are fused. In HDNET \cite{yang2018hdnet}, the semantics of HD maps and the 3D discretization of LIDAR 3D point clouds are concatenated and fed into a detection network, while in \cite{liang2018deep}, RGB features are fused into LIDAR BEV. Most importantly, BEV bridges the gap between perception and planning by preserving spatial relationships and abstracting most of the semantics needed for planning. Numerous approaches perform 3D object detection, object tracking, or motion prediction in BEV \cite{luo2018fast, yang2018pixor}, while planning models such as  learn directly from these simplified representations \cite{bansal2018chauffeurnet, wang2019monocular}. In this work, instead of predicting bounding boxes in BEV, we explore BEV in the form of bird's eye semantic segmentation. BE segmentation not only detects objects such as vehicles and pedestrians in finer details, but also predicts road lanes, stop signs, and sidewalks, providing planning models a more holistic view of the road scene.

\section{related works notes}

papers on planning using bird eys view
Chauffernet

introduce the task of be segmentation
mention mit paper, also should discuss that at the time of this writing, they didn't release their dataset, thus we collected a richer and more diverse dataset. emphaise more difficutl dataset

the use of depth information
most approaches only append depths as a channel
cornell paper shows that depth as an extra channel is not a convenient way for the model to learn
introduce pseudolidar
depth estimation

papers on simulator
GTAV simulator data paper
Carla simulator data paper

domain adaptation
domain adaptation papers
mention Muller's paper about the use of intermediate represetnation to minimize domain gap
mention instead of using side segmentation as intermediate representation, we use be pseudolidar as intermediate represetnation, this is agnostic not only to input rgb's brightness, glare, and other domain specific features, be pusedolidar is also agnostic to sensor counts and type(that is, lidar and radar could all contribute to this be pusedolidar)
